A Comprehensive and Reliable Feature Attribution Method: Double-sided Remove and Reconstruct (DoRaR)

The limited transparency of the inner decision-making mechanism in deep neural networks (DNN) and other machine learning (ML) models has hindered their application in several domains. In order to tackle this issue, feature attribution methods have been developed to identify the crucial features that heavily influence decisions made by these black box models. However, many feature attribution methods have inherent downsides. For example, one category of feature attribution methods suffers from the artifacts problem, which feeds out-of-distribution masked inputs directly through the classifier that was originally trained on natural data points. Another category of feature attribution method finds explanations by using jointly trained feature selectors and predictors. While avoiding the artifacts problem, this new category suffers from the Encoding Prediction in the Explanation (EPITE) problem, in which the predictor's decisions rely not on the features, but on the masks that selects those features. As a result, the credibility of attribution results is undermined by these downsides. In this research, we introduce the Double-sided Remove and Reconstruct (DoRaR) feature attribution method based on several improvement methods that addresses these issues. By conducting thorough testing on MNIST, CIFAR10 and our own synthetic dataset, we demonstrate that the DoRaR feature attribution method can effectively bypass the above issues and can aid in training a feature selector that outperforms other state-of-the-art feature attribution methods. Our code is available at https://github.com/dxq21/DoRaR.

==> Evaluating_improvement.tex <==
\section{Evaluating Improvement of Background Noise(BN), Reconstruction Loss(RL) and Complementary Mask(CM)}
\label{sec:evaluation1}

\subsection{Dataset and Experiment Setting}
\label{sec:Dataset and Experiment setting}

We test each improvement technique, e.g., including Bernoulli background noise, adding reconstruction loss, adding loss of complementary masked input as well as their combinations, in MNIST dataset, which includes 70000 28$\times$ 28 pixels images of hand written digits, 50000 for training, 10000 for validation and 10000 for testing respectively. A simple 2D CNN model is trained on the training set as the pre-trained classifier which achieves 93\% of test accuracy on the testing set. Our feature selector and generative model are built with 2D CNN and linear models respectively and are trained based on the pre-trained classifier and the same training set. For the details of the pre-trained classifier and DoRaR architectures, see Supplementary Materials S1.



\subsection{Testing Scheme}
We use the scheme shown in Fig.~\ref{fig:ts} to test all algorithms in this section and the next section. We choose this testing scheme for similar reasons as choosing our algorithm. Adding background noise can reduce the performance of the explanation that has EPITE problem. Showing results of both $a_1$ and $a_2$ can also reflect the EPTIE problem through high $a_2$. Most importantly, training a generative model to evaluate selected features rather than feeding masked images directly to the pre-trained classifier can prevent explanations that have the artifacts problem from getting unfair advantages over those explanations without the artifacts problem.


\subsection{Evaluated Methods}
\label{sec:Schemes and Metrics}
In order to prove the effectiveness of each improvement method, we compare every single improvement method, including adding the pixel-wise background noise, adding the reconstruction loss and adding the loss of complementary masked input as shown in Fig.~\ref{fig:tested improvements}. We compare each of them and all their combinations using the MNIST dataset.

\begin{figure}
\centering
    \subfigure[Baseline]{\label{fig:baseline}\includegraphics[width=\columnwidth]{baseline.jpg}}
\centering
    \subfigure[Baseline + Background Noise]{\label{fig:baseline+noise}\includegraphics[width=\columnwidth]{baseline+noise.jpg}}
\centering
    \subfigure[Baseline + Reconstruction Loss]{\label{fig:baseline+reconstructionloss}\includegraphics[width=\columnwidth]{baseline+reconstructionloss.jpg}}
\centering
    \subfigure[Baseline + Complementary Masked input]{\label{fig:baseline+complementarymask}\includegraphics[width=\columnwidth]{baseline+complementarymask.jpg}}
\centering
\caption{Diagrams of Improvement Methods}
%\vspace{-3mm}
\label{fig:tested improvements}
\end{figure}

We compare the performance of following the 8 schemes:
\begin{enumerate}
    \item B: Baseline \George{describe what baseline means.}\Dong{(Feature selector + Generative model without background noise, reconstruction loss and complementary masked input as shown in Fig.~\ref{fig:baseline}.)}
    \item BN: Baseline + Background Noise
    \item RL: Baseline + Reconstruction Loss
    \item CM: Baseline + Complementary Masked Input
    \item BN+RL: Baseline + Background Noise + Reconstruction Loss
    \item BN+CM: Baseline + Background Noise + Complementary Masked Input
    \item RL+CM: Baseline + Reconstruction Loss + Complementary Masked Input
    \item BN+RL+CM: Baseline + Background Noise + Reconstruction Loss + Complementary Masked Input(DoRaR)
\end{enumerate}
in terms of the accuracy $a_1$, the accuracy of the complementary masked input $a_2$, as shown in Fig.~\ref{fig:ts}.


\subsection{Results}
\label{subsec:self comparison results}
Fig.~\ref{fig:sctr} shows the results of all possible combinations of three improvement methods in selecting 4 chunks scenario and selecting 8 chunks scenario. The result shows the baseline always has the worst performance. Baseline combined with all three improvement methods has the best overall performance if we consider both $a_1$ and $a_2$. Single reconstruction loss has limited improvement, it has to be combined with other improvement methods. In the following section, we will compare our DoRaR algorithm that combines all three improvements with other algorithms.

